MAFIA: Machine Learning Acceleration on FPGAs for IoT Applications

Recent breakthroughs in ML have produced new classes of models that allow ML inference to run directly on milliwatt-powered IoT devices. On one hand, existing ML-to-FPGA compilers are designed for deep neural-networks on large FPGAs. On the other hand, general-purpose HLS tools fail to exploit properties specific to ML inference, thereby resulting in suboptimal performance. We propose MAFIA, a tool to compile ML inference on small form-factor FPGAs for IoT applications. MAFIA provides native support for linear algebra operations and can express a variety of ML algorithms, including state-of-the-art models. We show that MAFIA-generated programs outperform best-performing variant of a commercial HLS compiler by 2.5x on average.

==> figs/alg-opt.tex <==
\begin{algorithm}[t]
    \begin{algorithmic}[1]
	\caption{\textsc{Greedy DFG Optimization}}
	\label{alg:DFGOpt}
        \Function{DFGOpt}{\aA{DFG}, \aB{R\textsubscript{curr}}}
    		\While{\textsc{R}\textsubscript{curr} < \textsc{R}\textsubscript{total}}
        		\State Path\textsubscript{critical} $\gets$\Call {findCriticalPath} {DFG}
        		
        		\State Node\textsubscript{critical} $\gets$ \Call{findCriticalNode}{Path\textsubscript{critical}}
        		
        		\If{Node\textsubscript{critical} $\neq$ \texttt{None}}
        		    \State \textsc{R}\textsubscript{curr}, \textsc{DFG} $\gets$  \Call{UpdateDFG}{DFG, Node\textsubscript{critical}}
        		\Else
        		    \State break
        		\EndIf
        		
        	\EndWhile
        	\State \Return DFG 
    	\EndFunction
    	
    	
        \Function{findcriticalpath}{{DFG}}
            \State \textbf{var} latency\textsubscript{max}, Path\textsubscript{critical} $\gets -\infty$, []
            \State \textbf{var} paths $\gets$ \Call{getAllPaths}{DFG}
            \For{\texttt{path} in \textit{paths}}
                 \State \textbf{var} latency\textsubscript{currPath} $\gets$ \Call{getPathLatency}{\texttt{path}}
                \If{latency\textsubscript{currPath} $>$ latency\textsubscript{max}}
                    \State latency\textsubscript{max} $\gets$ latency\textsubscript{currPath}
                    \State Path\textsubscript{critical} $\gets$ \texttt{path}
                \EndIf
            \EndFor
            \State \Return Path\textsubscript{critical}, latency\textsubscript{max}
        \EndFunction
        
        
        \Function{findcriticalnode}{path}
            \State \textbf{var} gains $\gets$ \{\}
            \For{\texttt{node} in \textit{path}}
                \If{\Call{canUpdate}{node, DFG}} 
                    \State gains[node] $\gets$  $ \frac{Latency\textsubscript{old}- Latency\textsubscript{new} }  {Resource\textsubscript{new} - Resource\textsubscript{old} } $
                \Else
                    \State gains[node] $\gets -\infty$
                \EndIf
            \EndFor
             \Return node with max gain
        \EndFunction
		
	\Function{getallpaths}{path}
	    \State \texttt{//fetch all paths from \textbf{start} to \textbf{end}}
	    \State ......
	    \State \Return paths 
	\EndFunction
	
	\Function{canUpdate}{node, DFG}
	    \State \texttt{//determine whether increasing this node's PF by '1' is feasible}
	    \State ......
	\EndFunction
	
	\Function{updateDFG}{DFG, node}
	    \State DFG[node].PF += 1
	    \State \Return DFG
	\EndFunction
		
    \end{algorithmic}
\end{algorithm}


==> figs/codegen.tex <==
\begin{algorithm}[h]
    \begin{multicols}{2}
    
        \begin{algorithmic}
        
    	\caption{\textsc{Codegen Functions}}
    	    
    	    \State \textbf{struct} Mem $\{$
    	        \State \quad int size;
    	        \State \quad \textit{unsigned int}  Raddr, Waddr : $clog_2(size)$;
    	        \State \quad int Rdata, Wdata;
    	        \State \quad int Wen : 1;$\};$
    	    
            \Procedure{MatAdd}{A, B, $\mu$, $\rho$}
                \State PF, I, J $\gets$ $\rho[\mu]$, dim(A)
                \State \textbf{var} x[PF], y[PF], compute\_sizes[PF], $\mathit{offset}$
                \State  \textbf{Mem} C[PF]
                \State  \textbf{genvar} gi
                \State $\mathit{compute\_sizes}$, offset  $\gets$ \Call{getComputeSizes}{I, J, PF}
                \For{i in 0:PF}\Comment{\textit{initialize local memories}}
                    \State C[i] = \{.size = I*J/PF\}
                \EndFor
                
                \State \textbf{generate} begin
                \For{$\mathit{gi}$ in 0 : PF}
                    \For{$\mathit{addr}$ in 0 : compute\_sizes[gi]}
                         \State A[gi].Raddr $\gets$ addr+offset[gi],
                         \State B[gi].Raddr  $\gets$ addr+offset[gi]
                         \State x[gi], y[gi] $\gets$ A[gi].Rdata, B[gi].Rdata
                         \State C[gi].Wdata $\gets$ x[gi] + y[gi]
                         \State C[gi].Waddr $\gets$ addr+offset[gi]
                         \State C[gi].Wen $\gets$ 1
                    \EndFor
                \EndFor
                \State \textbf{endgenerate}
                \State \Return C
           \EndProcedure
           
           
        %   \Procedure{MatSub}{A, B, $\mu$, $\rho$}
        %         \State PF, I, J $\gets$ $\rho[\mu]$, dim(A)
        %         \State \textbf{var} x[PF], y[PF], compute\_sizes[PF]
        %         \State  \textbf{Mem} C[PF]
        %         \State  \textbf{genvar} gi
        %         \State $\mathit{compute\_sizes}$ $\gets$ \Call{getComputeSizes}{I, J, PF}
        %         \For{i in 0:PF}\Comment{\textit{initialize local memories}}
        %             \State C[i] = \{.size = I*J/PF\}
        %         \EndFor
                
        %         \State \textbf{generate} begin
        %         \For{$\mathit{gi}$ in 0 : PF}
        %             \For{$\mathit{addr}$ in 0 : compute\_sizes[gi]}
        %                  \State A[gi].Raddr, B[gi].Raddr  $\gets$ addr, addr
        %                  \State x[gi], y[gi] $\gets$ A[gi].Rdata, B[gi].Rdata
        %                  \State C[gi].Wdata $\gets$ x[gi] - y[gi]
        %                  \State C[gi].Waddr, C[gi].Wen $\gets$ addr, 1
        %             \EndFor
        %         \EndFor
        %         \State \textbf{endgenerate}
        %         \State \Return C
        %   \EndProcedure
           
            \Procedure{ScalarMul}{A, B, $\mu$, $\rho$}
                \State PF, I, J $\gets$ $\rho[\mu]$, dim(A)
                \State \textbf{var} x[PF], y[PF], compute\_sizes[PF], offset
                \State  \textbf{Mem} C[PF]
                \State  \textbf{genvar} gi
                \State $\mathit{compute\_sizes}$, offset  $\gets$ \Call{getComputeSizes}{I, J, PF}
                \For{i in 0:PF}\Comment{\textit{initialize local memories}}
                    \State C[i] = \{.size = I*J/PF\}
                \EndFor
                
                \State \textbf{generate} begin
                \For{$\mathit{gi}$ in 0 : PF}
                    \For{$\mathit{addr}$ in 0 : compute\_sizes[gi]}
                         \State B[gi].Raddr  $\gets$ addr+offset[gi]
                         \State x[gi], y[gi] $\gets$ A[0], B[gi].Rdata
                         \State C[gi].Wdata $\gets$ x[gi] + y[gi]
                         \State C[gi].Waddr $\gets$ addr+offset[gi]
                         \State C[gi].Wen $\gets$ 1
                    \EndFor
                \EndFor
                \State \textbf{endgenerate}
                \State \Return C
           \EndProcedure
           
           
           
        %   \Procedure{MulCir}{A, B, $\mu$, $\rho$}
        %         \State PF, I, J $\gets$ $\rho[\mu]$, dim(A)
        %         \State \textbf{var} x[PF], y[PF], compute\_sizes[PF]
        %         \State  \textbf{Mem} C[PF]
        %         \State  \textbf{genvar} gi
        %         \State $\mathit{compute\_sizes}$ $\gets$ \Call{getComputeSizes}{I, J, PF}
        %         \For{i in 0:PF}\Comment{\textit{initialize local memories}}
        %             \State C[i] = \{.size = I*J/PF\}
        %         \EndFor
                
        %         \State \textbf{generate} begin
        %         \For{$\mathit{gi}$ in 0 : PF}
        %             \For{$\mathit{addr}$ in 0 : compute\_sizes[gi]}
        %                  \State A[gi].Raddr, B[gi].Raddr  $\gets$ addr, addr
        %                  \State x[gi], y[gi] $\gets$ A[gi].Rdata, B[gi].Rdata
        %                  \State C[gi].Wdata $\gets$ x[gi] * y[gi]
        %                  \State C[gi].Waddr, C[gi].Wen $\gets$ addr, 1
        %             \EndFor
        %         \EndFor
        %         \State \textbf{endgenerate}
        %         \State \Return C
        %   \EndProcedure
           
           
           \Procedure{MatMul}{A, B, $\mu$, $\rho$}
                \If{I=1 and J=1 and K=1}
                    \State C[0] $\gets$ A[0] * B[0]
                \ElsIf{I=1 and J=1 and K$>$1}
                    \State \Return \Call{ScalarMul}{A, B, $\mu$, $\rho$}
                \ElsIf{I=1 and J$>$1 and K=1}
                    \State \Return \Call{mul-AddTree}{A, B, $\mu$, $\rho$}
                \ElsIf{I=1 and J$>$1 and K$>$1}
                    \State \Return \Call{vector-MatrixMM}{A, B, $\mu$, $\rho$}
                \ElsIf{I$>$1 and J=1 and K=1}
                    \State \Return \Call{ScalarMul}{B, A, $\mu$, $\rho$}
                \ElsIf{I$>$1 and J=1 and K$>$1}
                    \State \Return \Call{Vector-VectorMM}{A, B, $\mu$, $\rho$}
                \ElsIf{I$>$1 and J$>$1 and K=1}
                    \State \Return \Call{Matrix-VectorMM}{A, B, $\mu$, $\rho$}
                \ElsIf{I$>$1 and J$>$1 and K$>$1}
                    \State \Return \Call{Matrix-MatrixMM}{A, B, $\mu$, $\rho$}
                \EndIf
           \EndProcedure
           
           \vfill\null 
           \columnbreak
           
           \Procedure{Mul-AddTree}{A, B, $\mu$, $\rho$}
                \State PF, (I, J) $\gets$ $\rho[\mu]$, dim(A)
                \State \textbf{var} compute\_sizes[PF], offset[PF], acc[PF]
                \State  \textbf{Mem} C[PF]
                \State  \textbf{genvar} gi
                \State c\_sizes, offset $\gets$ \Call{getComputeSizes}{I, J, K, PF}
                \For{i in 0:PF}\Comment{\textit{initialize local memories}}
                    \State C[i] = \{.size = J/PF\}\Comment{distribute workload}
                \EndFor
                
                \State \textbf{generate} begin
                \For{$\mathit{gi}$ in 0:PF}
                    \State \textbf{var} maxSize $\gets$ compute\_sizes[gi] 
                    \State \textbf{var} x[maxSize], y[maxSize], z[maxSize] 
                    \For{$\mathit{addr}$ in 0 : maxSize}
                         \State A[gi].Raddr $\gets$ addr+offset[gi]
                         \State B[gi].Raddr $\gets$ addr+offset[gi] 
                         \State x[addr] $\gets$ A[gi].Rdata
                         \State y[addr] $\gets$ B[gi].Rdata
                         \State z[addr] $\gets$ x[addr] * y[addr]
                    \EndFor
                    \State \Call{AdderTree}{z, acc[gi]}
                \EndFor
                \State \textbf{endgenerate}
                \State \Call{AdderTree}{acc, C}\Comment{\textit{final Reduction tree}}
                \State \Return C
           \EndProcedure
           
           
           \Procedure{Vector-MatrixMM}{A, B, $\mu$, $\rho$}
                \State PF, (I, J), (J,K) $\gets$ $\rho[\mu]$, dim(A), dim(B)
                \State \textbf{var} compute\_sizes[PF], offset[PF], acc[PF]
                \State  \textbf{Mem} C[PF]
                \State  \textbf{genvar} gi
                \State c\_sizes, offset $\gets$ \Call{getComputeSizes}{I, J, K, PF}
                \For{i in 0:PF}\Comment{\textit{initialize local memories}}
                    \State C[i] = \{.size = J/PF\}\Comment{distribute workload}
                \EndFor
                \State \texttt{//transform A and B}
                \State \textbf{var} A\_trans $\gets$ \Call{Row-wisePartition}{A}
                \State \textbf{var} B\_trans $\gets$ \Call{Column-wisePartition}{B}
                
                \State \textbf{generate} begin
                \For{$\mathit{gi}$ in 0:PF}
                    \State \textbf{var} maxSize $\gets$ c\_sizes[gi] 
                    \State \textbf{var} x[maxSize], y[maxSize], z[maxSize] 
                    \For{$\mathit{addr}$ in 0 : maxSize}
                         \State A\_trans[gi].Raddr $\gets$ addr+offset[gi]
                         \State B\_trans[gi].Raddr $\gets$ addr+offset[gi] 
                         \State x[addr] $\gets$ A[gi].Rdata
                         \State y[addr] $\gets$ B[gi].Rdata
                         \State z[addr] $\gets$ x[addr] * y[addr]
                    \EndFor
                \EndFor
                \State \Call{Reduce}{z, C}\Comment{partial sum accumulation}
                \State \textbf{endgenerate}
                \State \Return C
           \EndProcedure
           
           
           
           
           


        	\Procedure{initzeros}{I, J}
        	    \State Mem T
        	    \State I, J $\gets$ dim(T)
        	    
        	    \If{I*J==1}
        	        \State \Return 
        	    \Else
        	        \For{i in 0:I}
                	    \For{j in 0:J}
                	        \State  T.Wdata $\gets$ 0
                             \State  T.Waddr $\gets$ i*I + j
                             \State  T.Wen $\gets$ 1 
                        \EndFor
                    \EndFor
                    \State  T.Wdata $\gets$ 0
                    \State  T.Waddr $\gets$ 0
                    \State  T.Wen $\gets$ 0
            	    \State \Return T
                \EndIf
        	\EndProcedure
        	
        	\Procedure{SGN}{x}
        	    \If{$x>0$}
        	        \State \Return 1
        	    \Else
        	        \State \Return 0
        	    \EndIf
        	\EndProcedure
        	
        \end{algorithmic}
    \end{multicols}
\end{algorithm}



==> figs/compilation_rules.tex <==
\section{Compilation Rules}

\subsection{Source Language}

\[

s ::= \tau x \quad\vert\quad  x = e \quad\vert\quad s_1; s_2 \quad\vert\quad \text{if(e) then } s_1 \text{else} s_2  \quad\vert\quad x=v

\tau ::= int \quad\vert\quad int[n] \quad\vert\quad int[n_1][n_2]   

e ::= x + y \quad\vert\quad x * y \quad\vert\quad x \geq  y \quad\vert\quad x \quad\vert\quad sgn(x) \quad\vert\quad tanh(x)

v ::= n \quad\vert\quad [n_1, ..., n_k] \quad\vert\quad [[n_1^1, ..., n_k^1], ....., [n_1^l, ..., n_k^l]]

\]


\subsection{Rules}
$\alpha$: mapping from variable name to memory name

$\Sigma$: mapping from memory name to memory content

$\Gamma$: mapping from variable name to Type($\tau$)

$\rho$: list of all variables that have been declared

$\mu$: mapping from matrix operation to instantiation name

$\kappa$: mapping from RAM to instantiation name

\[
\infer[C-Var]{
\vdash x \leadsto x
}
{
\begin{array}[b]{c}
\end{array}\quad
}
\]


\[
\infer[C-Assn]{
\vdash x  = e_2 \leadsto \textit{assign } d_1 = d_2;
}
{
\begin{array}[b]{c}
\vdash x \leadsto d_1 
\end{array}\quad
\begin{array}[b]{c}
\vdash e_2 \leadsto d_2 
\end{array}\quad
}
\]


\[
\infer[C-Add]{
\vdash e_1 + e_2 \leadsto d_1 + d_2
}
{
\begin{array}[b]{c}
\vdash e_1 \leadsto d_1 
\end{array}\quad
\begin{array}[b]{c}
\vdash e_2 \leadsto d_2 
\end{array}\quad
}
\]



\[
\infer[C-Mul]{
\vdash e_1 * e_2 \leadsto d_1 * d_2
}
{
\begin{array}[b]{c}
\vdash e_1 \leadsto d_1 
\end{array}\quad
\begin{array}[b]{c}
\vdash e_2 \leadsto d_2 
\end{array}\quad
}
\]


\[
\infer[C-GEQ]{
\vdash e_1 \geq e_2 \leadsto d_1 \geq d_2
}
{
\begin{array}[b]{c}
\vdash e_1 \leadsto d_1 
\end{array}\quad
\begin{array}[b]{c}
\vdash e_2 \leadsto d_2 
\end{array}\quad
}
\]


\[
\infer[C-Cond]{
 \rho \vdash \mathit{if}(e)\;then\;s_1\;else\;s_2 \leadsto C_1
}
{
\begin{array}[b]{c}
\vdash e \leadsto d 
\end{array}\quad
}
\]
 where, 

$C_1$ $\equiv$


\begin{lstlisting}[language=verilog]
always@* begin
    if(d)begin
        s_1;
    end
    else begin
        s_2;
    end
    
end

\end{lstlisting}
  


% \[
% \infer[C-Cond]{
%  \rho \vdash e_1 ? e_2 : e_3 \leadsto d_1 ? m_1 : m_2 || assign y_2 = d2; || delayChain_1 || assign y_3 = d_3; || delayChain_2, \rho
% }
% {
% \begin{array}[b]{c}
% D_1, D_2 = \textsc{GetDepth} (e_2, e_3) 
% \end{array}\quad
% \begin{array}[b]{c}
% \vdash e_1 \leadsto d_1 
% \end{array}\quad
% \begin{array}[b]{c}
% \vdash e_2 \leadsto d_2 
% \end{array}\quad
% \begin{array}[b]{c}
% \vdash e_3 \leadsto d_3 
% \end{array}\quad
% \begin{array}[b]{c}
% y_2 = fresh(\rho)
% \end{array}\quad
% \begin{array}[b]{c}
% y_3 = fresh(\rho)
% \end{array}\quad
% }
% \]
%  where, 

%   $delayChain_1 \leadsto delay \#(.DEPTH(D_1)) U\_D_1 (.clk(clk), .din(y_2), .dout(m_1)); $
 
%   $delayChain_2 \leadsto delay \#(.DEPTH(D_1)) U\_D_2 (.clk(clk), .din(y_3), .dout(m_2)); $



% \[
% \infer[C-Memory]{
% \alpha, \Sigma, \Gamma \vdash M \leadsto \Sigma[M], \alpha
% }
% {
% }
% \]

% where,

% C_1 \equiv RAM \#(.SIZE(I*J), .WIDTH(16))\quad \alpha[M]\quad (.clk(clk), .rst(rst),

% .Raddr(T_1.Raddr), .Rdata(T_1.Rdata), .Wdata(T_1.Wdata), .Waddr(T_1.Waddr), .Wen(T_1.Wen) );   

% \newline



\[
\infer[C-Matrix]{
\kappa, \Gamma, \alpha, \Sigma \vdash int[I][J]X  \leadsto \Sigma[T \mapsto k], \emptyset, \alpha[X \mapsto T], \Gamma[X \mapsto int[I][J]], \kappa'
}
{
\begin{array}[b]{c}
T = fresh(\Sigma)
\end{array}\quad
\begin{array}[b]{c}
k = initzeros(I, J, \kappa), \kappa'=\kappa+1
\end{array}\quad
}
\]


% \[
% \infer[C-Offset]{
% \kappa, \Gamma, \alpha, \Sigma \vdash int[I][J]X[offset]  \leadsto \Sigma[T \mapsto k], \emptyset, \alpha[X \mapsto T], \Gamma[X \mapsto int[I][J]], \kappa'
% }
% {
% \begin{array}[b]{c}
% T = fresh(\Sigma)
% \end{array}\quad
% \begin{array}[b]{c}
% k = initzeros(I, J), \kappa'=\kappa+1
% \end{array}\quad
% }
% \]


% \[
% \infer[C-Input]{
% \alpha, \Sigma \vdash input(X)  \leadsto Read(T)
% }
% {
% \begin{array}[b]{c}
% T = fresh(\Sigma)
% \end{array}\quad
% \begin{array}[b]{c}
% k = init(zeros, I, J)
% \end{array}\quad
% }
% \]

% \[
% \infer[C-Let]{
%     \vdash let x = e_1\;in\;e_2 \leadsto \emptyset 
% }
% {
% \begin{array}[b]{c}
% \vdash X \leadsto d_1
% \end{array}\quad
% \begin{array}[b]{c}
% \vdash e_1 \leadsto d_2
% \end{array}\quad
% \begin{array}[b]{c}
% \vdash e_2 \leadsto d_3
% \end{array}\quad
% }
% \]



\[
\infer[C-MatAdd]{
\kappa, \mu,\Sigma \vdash x + y \leadsto (T, \Sigma_1, MatAdd_\mu(T_1, T_2, T)), \mu' 
}
{
\begin{array}[b]{c}
T_1 = \alpha(x)
\end{array}\quad
\begin{array}[b]{c}
T_1 = \alpha(y)
\end{array}\quad
\begin{array}[b]{c}
\mu'=\mu+1,
T=fresh(\Sigma),
k=initzeros(I,J,\kappa),
\Sigma_1 = \Sigma[T \mapsto k]
\end{array}\quad
}
\]

\[
\infer[C-MatMul]{
\kappa, \mu,\Sigma \vdash x * y \leadsto (T, \Sigma_1, MatMul_\mu(T_1, T_2, T)), \mu' 
}
{
\begin{array}[b]{c}
T_1 = \alpha(x)
\end{array}\quad
\begin{array}[b]{c}
T_1 = \alpha(y)
\end{array}\quad
\begin{array}[b]{c}
\mu'=\mu+1,
T=fresh(\Sigma),
k=initzeros(I,J,\kappa),
\Sigma_1 = \Sigma[T \mapsto k]
\end{array}\quad
}
\]

\[
\infer[C-MulCir]{
\kappa, \mu,\Sigma \vdash x <*> y \leadsto (T, \Sigma_1, MulCir_\mu(T_1, T_2, T)), \mu' 
}
{
\begin{array}[b]{c}
T_1 = \alpha(x)
\end{array}\quad
\begin{array}[b]{c}
T_1 = \alpha(y)
\end{array}\quad
\begin{array}[b]{c}
\mu'=\mu+1,
T=fresh(\Sigma),
k=initzeros(I,J,\kappa),
\Sigma_1 = \Sigma[T \mapsto k]
\end{array}\quad
}
\]

\[
\infer[C-SparseMatMul]{
\kappa, \mu,\Sigma \vdash x |*| y \leadsto (T, \Sigma_1, SparseMatMul_\mu(T_1, T_2, T)), \mu' 
}
{
\begin{array}[b]{c}
T_1 = \alpha(x)
\end{array}\quad
\begin{array}[b]{c}
T_1 = \alpha(y)
\end{array}\quad
\begin{array}[b]{c}
\mu'=\mu+1,
T=fresh(\Sigma),
k=initzeros(I,J,\kappa),
\Sigma_1 = \Sigma[T \mapsto k]
\end{array}\quad
}
\]



\[
\infer[C-TanH]{
\mu,\Sigma \vdash tanh(x) \leadsto (T, \Sigma_1, TanH_\mu(T_1, T)), \mu' 
}
{
\begin{array}[b]{c}
\Sigma \vdash e \leadsto (T_1, \Sigma)
\end{array}\quad
\begin{array}[b]{c}
\mu'=\mu+1,
T=fresh(\Sigma),
k=initzeros(I,J),
\Sigma_1 = \Sigma[T \mapsto k], \Gamma[x] = int[I][J]
\end{array}\quad
}
\]


\[
\infer[C-SGN]{
\mu \vdash sgn(x) \leadsto (SGN_\mu(x)), \mu' 
}
{
\begin{array}[b]{c}
\Sigma \vdash x \leadsto x
\end{array}\quad
\begin{array}[b]{c}
\mu'=\mu+1, \Gamma[x] = int
\end{array}\quad
}
\]







% \begin{algorithm}[H]
%     \begin{algorithmic}
% 	\caption{\textsc{Auxiliary Functions}}
%         \Function{GetDepth}{\aA{e\textsubscript{1}}, \aB{e\textsubscript{2}}}
            
%             \State \textbf{latency\textsubscript{e\textsubscript{1}}} $\gets$ 0
%             \State \textbf{latency\textsubscript{e\textsubscript{2}}} $\gets$ 0
%     		\For{\texttt{op} in \textit{e\textsubscript{1}}}
%                  \State \textbf{latency\textsubscript{e\textsubscript{1}}}  $\gets$ \textbf{latency\textsubscript{e\textsubscript{1}}} + \Call{GetLatency}{\texttt{op}}
%             \EndFor
            
%             \For{\texttt{op} in \textit{e\textsubscript{2}}}
%                  \State \textbf{latency\textsubscript{e\textsubscript{2}}}  $\gets$ \textbf{latency\textsubscript{e\textsubscript{2}}} + \Call{GetLatency}{\texttt{op}}
%             \EndFor
            
%             \If{latency\textsubscript{e\textsubscript{1}} $\geq$ latency\textsubscript{e\textsubscript{2}}}
%                 \State \Return 0, \abs{latency\textsubscript{e\textsubscript{1}} - latency\textsubscript{e\textsubscript{2}} }
%             \Else
%                 \State \Return \abs{latency\textsubscript{e\textsubscript{2}} - latency\textsubscript{e\textsubscript{1}} }, 0
%             \EndIf
    		
%     	\EndFunction
    	
%     	\Function{GetLatency}{\aA{Op}}
%     		\If{\textsc{Op} $==$ \textsc{'*'} }
%         		\State \Return 3 
%         	\EndIf
%         	\If{\textsc{Op} $==$ \textsc{'+'}}
%         	    \State \Return 2
%         	\EndIf
        	 
%         	\State \Return 0
        		
%     	\EndFunction
    	
    	
%     \end{algorithmic}
% \end{algorithm}






==> figs/table-baseline-latency.tex <==
\begin{table*}[t]
\centering
\small

% \begin{tabular}{|| c | c | c | c | c | c | c | c | c | c | c ||}
\begin{tabular}{ccccccccccc}

 \textbf{DATASET} & cifar-b & cr-b & mnist-b & usps-b & ward-b & cr-m & curet-m & letter-m & mnist-m & usps-m\\ 
 \hline
  \textbf{Num Features}& 6 & 87837 & 787 \\ 

 \hline
 \textbf{Baseline latency (us)} & 1 & 1 % 
\end{tabular}

\caption{Table to test captions and labels}
\label{table-new}
\end{table*}
